6GCVAE: Gated Convolutional Variational Autoencoder for IPv6 Target Generation

IPv6 scanning has always been a challenge for researchers in the field of network measurement. Due to the considerable IPv6 address space, while recent network speed and computational power have been improved, using a brute-force approach to probe the entire network space of IPv6 is almost impossible. Systems are required an algorithmic approach to generate more possible active target candidate sets to probe. In this paper, we first try to use deep learning to design such IPv6 target generation algorithms. The model effectively learns the address structure by stacking the gated convolutional layer to construct Variational Autoencoder (VAE). We also introduce two address classification methods to improve the model effect of the target generation. Experiments indicate that our approach 6GCVAE outperformed the conventional VAE models and the state-of-the-art target generation algorithm in two active address datasets.

==> PAKDD 2020/.git/objects/13/c60964e1eb72855d187876a21162bb06ee226f <==
x]'OkÃ0Åwä;èض±õ°ãZƒP-cWÇQ3Ç6²²¶ß~Vþ@·å÷¤ß"RY_Áófs³CEP–û톈t›gyvìc1'qÀ‰PB͞.P¡õ®öé¡TGüzDJ«6¹<åY™¤!ì=O-¶¾#ÁAta%óÖà82®EºûD²ª-dü;ƒö.šÈQ$2§ñÖúSRN\/" TuŸ–o¤öI'Ø…úZ"í~¢ñæçeʜb²Zët,´Kkø"¸özèÑ%T«bœ,QõÁbP©`<‹QÁTLJUnLûP`¸j›D©(K¨§ã?Ÿ8G¢4·u3CI˜…D±Dš6RÁêc÷¶"]όArÝ?U\¶¦"I2þ¯¦J'…È‹p2܁²¡S²Ñ=q:Bžý?µ

==> PAKDD 2020/.git/objects/45/d2d389f2a92416d112df75251b766227d79096 <==
xŽK
1D]çÙÒIO:¼'HÒ-Îb>"dáí<'Ô¦xŃªÛ²ÌÝzô§ÞTm….½\,% ùHǞ‹LŒ9˜=7]»U_Kô€Z¥È%¤¨™Ä×	˜"II
›<ú{kö1æçœ×Ï°×:æþ«‰ Üá¥nËͺñ3Û30€9èq²ëŸº»ä®¶i–EÍdÄFx
